On Improving Adversarial Transferability of Vision Transformers

Vision transformers (ViTs) process input images as sequences of patches via self-attention; a radically different architecture than convolutional neural networks (CNNs). This makes it interesting to study the adversarial feature space of ViT models and their transferability. In particular, we observe that adversarial patterns found via conventional adversarial attacks show very \emph{low} black-box transferability even for large ViT models. We show that this phenomenon is only due to the sub-optimal attack procedures that do not leverage the true representation potential of ViTs. A deep ViT is composed of multiple blocks, with a consistent architecture comprising of self-attention and feed-forward layers, where each block is capable of independently producing a class token. Formulating an attack using only the last class token (conventional approach) does not directly leverage the discriminative information stored in the earlier tokens, leading to poor adversarial transferability of ViTs. Using the compositional nature of ViT models, we enhance transferability of existing attacks by introducing two novel strategies specific to the architecture of ViT models. (i) Self-Ensemble: We propose a method to find multiple discriminative pathways by dissecting a single ViT model into an ensemble of networks. This allows explicitly utilizing class-specific information at each ViT block. (ii) Token Refinement: We then propose to refine the tokens to further enhance the discriminative capacity at each block of ViT. Our token refinement systematically combines the class tokens with structural information preserved within the patch tokens.

==> figures/DIM_table.tex <==
% \begin{table}[]
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
%                               & Res152    & WRN               & DN201       & T2T-7       & T2T-24       & TnT        & ViT-S & ViT-L      \\ \hline
% % densenet121                   & 85.1      & 87.92             & 92.6        & 68.86       & 46.22        & 49.2                 \\ \hline
% vgg19                         & 62.08     & 68.30             & 73.48       & 58.62       & 30.16        & 34.70      &35.42  &	16.86            \\ \hline
% mnasnet1\_0                   & 68.3      & 70.06             & 77.18       & 71.98       & 42.92        & 47.24      &52.74  &	25.06           \\ \hline
% tiny\_patch16\_224            & 65.48     & 65.62             & 72.68       & 86.4        & 70.16        & 82.68      &89.16  &	62.00           \\ \hline
% tiny\_patch16\_224\_ensemble  & 70.78     & 70.78             & 78.4        & 91.08       & 68.56        & 84.18      &93.36  &	67.58           \\ \hline
% small\_patch16\_224           & 62.12     & 63.42             & 67.3        & 74.34       & 73.84        & 79.5       &82.32  &	62.62           \\ \hline
% small\_patch16\_224\_ensemble & 81.3      & 82.64             & 86.98       & 93.88       & 85.26        & 93.22      &96.56  &	78.88           \\ \hline
% base\_patch16\_224            & 59.14     & 60.64             & 64.44       & 67.28       & 69.54        & 73.96      &76.32  &	61.38           \\ \hline
% base\_patch16\_224\_ensemble  & 84.92     & 86.36             & 89.24       & 92.36       & 84.0         & 92.28      &95.26  &	78.90           \\ \hline
% \end{tabular}
% \caption{DIM table at eps-16}
% \label{tab:dim_adv}
% \end{table}


\begin{table}[!t]
	\centering\small
% 		\setlength{\tabcolsep}{2pt}
		\scalebox{1.0}[1.0]{
		\begin{tabular}{ @{\extracolsep{\fill}} l|l|ccc|ccccc}
				\toprule
			& &  \multicolumn{3}{c}{Convolutional} & \multicolumn{5}{c}{Transformers}   \\
			\cline{3-10}
			\multirow{-3}{*}{Source} &\multirow{-3}{*}{Attack}& {Res152} & {WRN} & DN201 & {ViT-L} &  {T2T-24} & {TnT} & {VIT-S} & {T2T-7}\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{VGG19$_{bn}$}} & DIM & 62.08 & 68.30  & 73.48 &16.86& 30.16  & 34.70 &35.42& 58.62  \\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{MNAS}} & DIM & 62.08 & 68.30  & 73.48 &	25.06 & 42.92& 47.24 & 52.74 & 71.98  \\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-T}} & DIM & 68.3  & 70.06 & 77.18 & 62.00& 70.16& 82.68 & 89.16& 72.68  \\
			& DIM$^{E}$ & \\
			& DIM$^{RE}$ & 70.78 & 70.78  & 78.4 & 67.58& 68.56  & 84.18&93.36& 78.4  \\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-S}} & DIM & 62.12 & 63.42 & 67.30 & 62.62& 73.84& 79.5 & 82.32& 67.3\\
			& DIM$^{E}$ & \\
			& DIM$^{RE}$ & 81.30& 82.64  & 86.98 &78.88& 85.26  & 93.22&96.56  & 86.98 \\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-B}} & DIM &59.14  & 60.64 & 64.44&	61.38 & 69.54& 73.96 & 76.32& 64.44   \\
			& DIM$^{E}$ & \\
			& DIM$^{RE}$ & 84.92 & 86.36 & 89.24&	78.90& 84.0 & 92.28 & 95.26 & 89.24 \\
			\midrule
			\bottomrule
	\end{tabular}}
	\caption{\emph{\textbf{Adversarial Transferability:}} Fool rate (\%) on 5k ImageNet val. samples. Perturbation budget: $l_\infty \le 16$. Adversarial perturbations generated from hierarchical-ensemble of a single vision transformer have significantly higher transferability for a given adversarial attacks.}
	\label{tab:transferability-h-ensemble}
\end{table}


==> figures/PGD_table.tex <==
\begin{table}[!t]
	\centering\small
% 		\setlength{\tabcolsep}{2pt}
		\scalebox{1.0}[1.0]{
		\begin{tabular}{ @{\extracolsep{\fill}} l|l|ccc|ccccc}
				\toprule
			& &  \multicolumn{3}{c}{Convolutional} & \multicolumn{5}{c}{Transformers}   \\
			\cline{3-10}
			\multirow{-3}{*}{Source} &\multirow{-3}{*}{Attack}& {Res152} & {WRN} & DN201 & {ViT-L} &  {T2T-24} & {TnT} & {VIT-S} & {T2T-7}\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{VGG19$_{bn}$}} & PGD & 28.56 & 33.92 & 33.22 & 5.94 & 10.78 & 12.96 & 13.08 & 29.90\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{MNAS}} & PGD & 36.28 & 36.22 & 40.20 & 8.04 & 18.04 & 21.16 & 19.60 & 41.70\\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-T}} & PGD & 23.98 & 24.16 & 26.76 & 35.70 & 21.54 & 44.24 & 86.86 & 53.74 \\
			& PGD$^{E}$ & 24.58 & 25.46 & 28.38 & 39.84 & 21.86 & 45.08 & 88.44 & 53.80\\
			& PGD$^{RE}$ & 34.64 & 37.62 & 40.56 & 58.6 & 26.58 & 55.52 & 96.34 & 66.68\\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-S}} & PGD & 24.96 & 26.38 & 30.38 & 37.84 & 33.46 & 60.62 & 84.38 & 52.76\\
			& PGD$^{E}$ & 27.72 & 29.54 & 32.90 & 44.30 & 35.4 & 64.76 & 89.82 & 52.76\\
			& PGD$^{RE}$ & 38.92 & 42.84 & 46.82 & 60.86 & 40.3 & 76.10 & 97.32 & 71.54\\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-B}} & PGD & 25.56 & 27.90 & 30.24 & 34.08 & 31.98 & 52.76 & 69.82 & 39.80\\
			& PGD$^{E}$ & 32.84 & 35.40 & 38.66 & 43.56 & 37.82 & 64.20 & 82.32 & 51.68\\
			& PGD$^{RE}$ & 49.10 & 53.38 & 56.96 & 56.9 & 45.7 & 79.56 & 94.10 & 74.78\\
			\midrule
			\bottomrule
	\end{tabular}}
	\caption{\emph{\textbf{Adversarial Transferability:}} Fool rate (\%) on 5k ImageNet val. samples. Perturbation budget: $l_\infty \le 16$. Adversarial perturbations generated from hierarchical-ensemble of a single vision transformer have significantly higher transferability for a given adversarial attacks.}
	\label{tab:transferability-h-ensemble}
\end{table}


==> figures/Untarget_TI.tex <==
\begin{table}[t]
	\centering\small
\setlength{\tabcolsep}{2pt}
		\scalebox{0.93}[0.93]{
		\begin{tabular}{ @{\extracolsep{\fill}} l|l|lll|lllll@{}}
        \toprule[0.3mm]
			\rowcolor{Gray} 
			\multicolumn{10}{c}{\small \textbf{Translation-Invariant (TI) \cite{dong2019evading}  }} \\ \midrule[0.3mm]
						& &  \multicolumn{3}{c}{Convolutional} & \multicolumn{5}{c}{Transformers}   \\
			\cmidrule{3-10}
			\multirow{-3}{*}{Source ($\downarrow$)} &\multirow{-3}{*}{Attack}& {Res152} & {WRN} & DN201 & {ViT-L} &  {T2T-24} & {TnT} & {ViT-S} & {T2T-7}\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{VGG19$_{bn}$}} & TI-DIM & 54.54 & 64.06 & 62.58 & 28.22 & 17.56 & 20.16 & 36.78 & 43.08 \\ 
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{MNAS}} & TI-DIM & 55.44 & 62.84 & 65.36 & 35.80  & 22.24 & 25.26 & 46.16 & 48.80  \\ 
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-T}} & TI-DIM & 49.96 & 56.02 & 57.08 & 53.24 & 37.76 & 50.90  & 72.20  & 66.32 \\
			& TI-DIM$^{E}$ & 52.32 & 60.02 & 60.82 & 57.82 & 37.00 & 50.34 & 75.20  & 68.18 \\
			& TI-DIM$^{RE}$ & 51.70\inc{1.74} & 60.32\inc{4.30} & 61.46\inc{4.38} & 55.06\inc{1.82} & 32.74\dec{5.02} & 45.60\dec{5.30} & 72.80\inc{0.60} & 65.82\dec{0.50} \\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-S}} & TI-DIM & 47.44 & 53.24 & 52.94 & 54.64 & 47.70  & 58.76 & 67.48 & 53.32 \\
			& TI-DIM$^{E}$ & 54.96 & 61.12 & 61.94 & 65.10  & 50.74 & 63.72 & 78.54 & 62.66 \\
			& TI-DIM$^{RE}$ & 59.20\inc{11.76} & 66.54\inc{13.30} & 67.30\inc{14.36} & 66.54\inc{11.90} & 46.56\dec{1.14} & 60.30\inc{1.54} & 79.86\inc{12.38} & 67.78\inc{14.46} \\
			\midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-B}} & TI-DIM & 44.90  & 51.16 & 50.14 & 53.46 & 44.7  & 51.60  & 60.24 & 44.06 \\
			& TI-DIM$^{E}$ & 56.44 & 64.30  & 63.70  & 67.48 & 50.84 & 60.92 & 76.94 & 57.94 \\
			& TI-DIM$^{RE}$ & 61.92\inc{17.02} & 70.36\inc{19.20} & 71.60\inc{21.46} & 67.78\inc{14.32} & 46.18\inc{1.48} & 58.28\inc{6.68} & 78.24\inc{18.00} & 65.80\inc{21.74} \\
			
			\bottomrule[0.3mm]
	\end{tabular}}
	\caption{\emph{\textbf{Fool rate (\%)}} on 5k ImageNet val. adversarial samples at $l_\infty \le 16$. Perturbations generated from our proposed ensemble of refined token from a vision transformer have significantly higher success rate.}
	\label{tab:ut_ti}
\end{table}


==> figures/adversarial_dim.tex <==
\begin{table}[h]
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\toprule[0.3mm]
\rowcolor{Gray} 
\multicolumn{9}{c}{\small \textbf{Translation Invariance \cite{dong2019evading} with Input Diversity (DIM) \cite{xie2019improving}}} \\ \midrule[0.3mm]

\multirow{3}{*}{Models}           & \multicolumn{4}{c|}{$l_\infty \le 8$}  & \multicolumn{4}{c}{$l_\infty \le 16$} \\ \cmidrule{2-9} 
 &
  \multicolumn{2}{c|}{ResNet18} &
  \multicolumn{2}{c|}{ResNet50} &
  \multicolumn{2}{c|}{ResNet18} &
  \multicolumn{2}{c }{ResNet50} \\ \cmidrule{2-9} 
 &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l}{$\epsilon = 8$} \\ \midrule

% VGG19$_{bn}$    & 16.9  & 15    & 16.38 & 13.26 & 38.88 & 35.38 & 37.92 & 32.32 \\ \hline
% MNAS            & 17.42 & 15.44 & 17.18 & 13.9  & 40.36 & 36.1  & 39.08 & 33.34 \\ \hline
% DeiT-T          & 17.78 & 15.56 & 18.34 & 14.28 & 40.94 & 36.94 & 40.26 & 34.04 \\ \hline
% DeiT-T-RE       & 20    & 16.82 & 20.14 & 15.36 & 43.08 & 38.34 & 43.5  & 35.82 \\ \hline
% DeiT-S          & 17.64 & 15.52 & 17.5  & 14.08 & 40.06 & 36.5  & 39.18 & 33.42 \\ \hline
% DeiT-S-RE       & 19.9  & 16.72 & 20.58 & 16.06 & 43.48 & 38.9  & 43.46 & 35.9  \\ \hline
% DeiT-B          & 18.14 & 16.36 & 17.42 & 14.3  & 40.1  & 37.14 & 39.56 & 34.12 \\ \hline
% DeiT-B-RE       & 20.72 & 17.38 & 21.08 & 16.54 & 44.52 & 39.7  & 45.84 & 37.22 \\ \hline

VGG19$_{bn}$    & 20.7  & 17.3  & 20.54 & 16.24 & 46.06 & 40.28 & 46.1  & 40.02 \\ \midrule
MNAS            & 21.56 & 17.1  & 20.9  & 16.4  & 46.8  & 40.18 & 46.68 & 39.9  \\ \midrule
DeiT-T          & 21.22 & 17.34 & 21.42 & 16.3  & 47.1  & 40.7  & 46.44 & 40.78 \\ 
DeiT-T-RE       & 23.7  & 19.44 & 23.7  & 18.32 & 50.5  & 43.14 & 50.84 & 43.62 \\ \midrule
DeiT-S          & 20.78 & 16.74 & 19.84 & 15.88 & 46.06 & 39.52 & 45.1  & 38.84 \\ 
DeiT-S-RE       & 23.44 & 19.82 & 24.02 & 18.52 & 50.64 & 43.34 & 51.12 & 43.5  \\ \midrule
DeiT-B          & 21.1  & 17.06 & 20.42 & 15.98 & 46.3  & 41.04 & 45.3  & 38.4  \\ 
DeiT-B-RE       & 25.02 & 20.64 & 24.56 & 18.94 & 52.02 &       & 52.34 & 44.72 \\ \midrule


\end{tabular}
\caption{Untargetted Attack on Adversarially trained models \cite{salman2020adversarially}}
\label{tab:tar_dim}
\end{table}

==> figures/adversarial_mim.tex <==
\begin{table}[]
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
\multirow{3}{*}{Models}           & \multicolumn{4}{c|}{$l_\infty \le 8$}  & \multicolumn{4}{c}{$l_\infty \le 16$} \\ \cline{2-9} 
 &
  \multicolumn{2}{c|}{ResNet18} &
  \multicolumn{2}{c|}{ResNet50} &
  \multicolumn{2}{c|}{ResNet18} &
  \multicolumn{2}{c }{ResNet50} \\ \cline{2-9} 
 &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l|}{$\epsilon = 8$} &
  \multicolumn{1}{l|}{$\epsilon = 4$} &
  \multicolumn{1}{l }{$\epsilon = 8$} \\ \hline

VGG19$_{bn}$    & 16.24           & 14.88           & 15.56           & 13.32           & 36.16            & 31.68            & 38.04            & 34.5             \\ \hline
MNAS            & 16.88           & 14.84           & 16.18           & 13.28           & 37.24            & 32.1             & 38.86            & 35.16            \\ \hline
DeiT-T          & 17.94           & 16.08           & 17.6            & 14.46           & 39.48            & 33.96            & 40.5             & 36.28            \\ \hline
DeiT-T-RE       & 19.58           & 16.56           & 19.22           & 15.14           & 41.88            & 35.06            & 41.46            & 37.42            \\ \hline
DeiT-S          & 18.64           & 15.96           & 17.1            & 14.14           & 38.86            & 33.56            & 39.84            & 36.74            \\ \hline
DeiT-S-RE       & 20.48           & 17.18           & 20.04           & 15.36           & 42.48            & 35.4             & 42.72            & 37.94            \\ \hline
DeiT-B          & 18.14           & 16.0            & 16.98           & 14.56           & 39.24            & 33.5             &                  &                  \\ \hline
DeiT-B-RE       & 20.12           & 17.54           & 19.96           & 15.9            & 43.92            &                  &                  &                  \\ \hline

\end{tabular}
\caption{Untargetted Attack: MIM}
\label{tab:tar_mim}
\end{table}


==> figures/detr_vis.tex <==
\begin{figure}[t]
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/1vis_orig.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/3vis_orig.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/5vis_orig.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/7vis_orig.jpg}
    \end{minipage}
    %
    \begin{minipage}{\textwidth}
        \centering
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/1vis_adv.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/3vis_adv.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/5vis_adv.jpg}
        \includegraphics[width=0.24\linewidth, height=2cm]{figures/detr_vis/7vis_adv.jpg}

    \end{minipage}
\end{figure}

==> figures/dino_vis.tex <==
\begin{figure}[h]
    \begin{minipage}{0.4\textwidth}
    \includegraphics[width=\linewidth]{figures/plots/dino.png}
    \caption{We quantitatively measure the variation of attention map quality against varying attack strength (max. perturbation) for MI-FGSM using segmentation evaluation approach from DINO \citep{caron2021emerging}. The attacks successfully alter the attention of models.}
    \label{fig:dino_vis}
    \end{minipage}
    \hspace{0.02\textwidth}
    \begin{minipage}{0.58\textwidth}
        \begin{minipage}{\textwidth}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/1good.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/7good.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/6good.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/4good.jpg}
        \end{minipage}
        %
        \begin{minipage}{\textwidth}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/1adv.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/7adv.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/6adv.jpg}
        \includegraphics[width=0.24\linewidth]{figures/attn_vis/4adv.jpg}
        \end{minipage}
    \captionof{figure}{Qualitative results for effect of attacks on attention of VIT models. We use a pre-trained DINO \citep{caron2021emerging} model and visualize the altered attention maps (below) due to our attack.}
    \end{minipage}
\end{figure}

==> figures/target_DIM.tex <==
\begin{table}[t]
	\centering\small
% 		\setlength{\tabcolsep}{2pt}
\setlength{\tabcolsep}{2pt}
		\scalebox{1}[1]{
		\begin{tabular}{ @{\extracolsep{\fill}} l|l|lll|lllll@{}}
        \toprule[0.3mm]
        \rowcolor{Gray} 
        \multicolumn{10}{c}{\small \textbf{DIM Targeted Attack \cite{dong2018boosting}}} \\ \midrule[0.3mm]
			& &  \multicolumn{3}{c}{Convolutional} & \multicolumn{5}{c}{Transformers}   \\
			\cmidrule{3-10}
			\multirow{-3}{*}{Source ($\downarrow$)} &\multirow{-3}{*}{Attack}& {Res152} & {WRN} & DN201 & {ViT-L} &  {T2T-24} & {TnT} & {ViT-S} & {T2T-7}\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{VGG19$_{bn}$}} & MIM & 0.29 & 0.40 & 0.61 & 0.11 & 0.15 & 0.16  & 0.12  & 0.29  \\ \midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{MNAS}}         & MIM & 0.42 & 0.40 & 0.76 & 0.11 & 0.27 & 0.26  & 0.21  & 0.63  \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-T}}       & MIM & 0.22 & 0.19 & 0.33 & 0.74 & 0.49 & 1.70  & 20.44 & 1.24  \\
			                                                       & MIM$^{RE}$ & 0.50\inc{0.28} & 0.50\inc{0.31} & 1.12\inc{0.79} & 3.08\inc{2.34} & 1.09\inc{0.60} & 6.46\inc{4.76} & 55.21\inc{34.77} & 6.12\inc{4.88}  \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-S}}       & MIM & 0.20 & 0.19 & 0.31 & 0.67 & 0.73 & 2.45  & 8.31  & 0.81  \\
			                                                       & MIM$^{RE}$ & 0.89\inc{0.69} & 0.93\inc{0.74} & 2.05\inc{1.74} & 4.90\inc{4.23} & 3.57\inc{2.84} & 21.56\inc{19.11} & 64.65\inc{56.34} & 10.59\inc{9.78} \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-B}}       & MIM & 0.23 & 0.21 & 0.35 & 0.60 & 0.71 & 1.89  & 4.14  & 0.62  \\
			                                                       & MIM$^{RE}$ & 1.13\inc{0.90} & 1.22\inc{1.01} & 2.65\inc{2.30} & 3.59\inc{2.99} & 3.45\inc{2.74} & 17.55\inc{15.66} & 44.63\inc{40.49} & 9.89\inc{9.27} \\ \bottomrule[0.3mm]
	\end{tabular}}\vspace{0.5em}
	\caption{{\textbf{Fool rate (\%)}} on 5k ImageNet val. for adversarial samples at $\epsilon \le 16$ generated using targeted attack (using average over 10 targets). Perturbations generated from our proposed self-ensemble with refined tokens exhibit have a higher success rate. \knr{values wrong - to be updated}}
	\label{tbl:targetted_dim}
\end{table}


==> figures/target_MIM.tex <==
\begin{table}[t]
	\centering\small
% 		\setlength{\tabcolsep}{2pt}
\setlength{\tabcolsep}{2pt}
		\scalebox{1}[1]{
		\begin{tabular}{ @{\extracolsep{\fill}} l|l|lll|lllll@{}}
        \toprule[0.3mm]
        \rowcolor{Gray} 
        \multicolumn{10}{c}{\small \textbf{MIM Targeted Attack \cite{dong2018boosting}}} \\ \midrule[0.3mm]
			& &  \multicolumn{3}{c}{Convolutional} & \multicolumn{5}{c}{Transformers}   \\
			\cmidrule{3-10}
			\multirow{-3}{*}{Source ($\downarrow$)} &\multirow{-3}{*}{Attack}& {Res152} & {WRN} & DN201 & {ViT-L} &  {T2T-24} & {TnT} & {ViT-S} & {T2T-7}\\
			\midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{VGG19$_{bn}$}} & MIM & 0.29 & 0.40 & 0.61 & 0.11 & 0.15 & 0.16  & 0.12  & 0.29  \\ \midrule
			\multirow{1}{*}{\rotatebox[origin=c]{0}{MNAS}}         & MIM & 0.42 & 0.40 & 0.76 & 0.11 & 0.27 & 0.26  & 0.21  & 0.63  \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-T}}       & MIM & 0.22 & 0.19 & 0.33 & 0.74 & 0.49 & 1.70  & 20.44 & 1.24  \\
			                                                       & MIM$^{RE}$ & 0.50\inc{0.28} & 0.50\inc{0.31} & 1.12\inc{0.79} & 3.08\inc{2.34} & 1.09\inc{0.60} & 6.46\inc{4.76} & 55.21\inc{34.77} & 6.12\inc{4.88}  \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-S}}       & MIM & 0.20 & 0.19 & 0.31 & 0.67 & 0.73 & 2.45  & 8.31  & 0.81  \\
			                                                       & MIM$^{RE}$ & 0.89\inc{0.69} & 0.93\inc{0.74} & 2.05\inc{1.74} & 4.90\inc{4.23} & 3.57\inc{2.84} & 21.56\inc{19.11} & 64.65\inc{56.34} & 10.59\inc{9.78} \\ \midrule
			\multirow{3}{*}{\rotatebox[origin=c]{0}{Deit-B}}       & MIM & 0.23 & 0.21 & 0.35 & 0.60 & 0.71 & 1.89  & 4.14  & 0.62  \\
			                                                       & MIM$^{RE}$ & 1.13\inc{0.90} & 1.22\inc{1.01} & 2.65\inc{2.30} & 3.59\inc{2.99} & 3.45\inc{2.74} & 17.55\inc{15.66} & 44.63\inc{40.49} & 9.89\inc{9.27}  \\ \bottomrule[0.3mm]
	\end{tabular}}\vspace{0.5em}
	\caption{{\textbf{Fool rate (\%)}} on 5k ImageNet val. for adversarial samples at $\epsilon \le 16$ generated using targeted attack (using average over 10 targets). Perturbations generated from our proposed self-ensemble with refined tokens exhibit have a higher success rate.}
	\label{tbl:targetted_mim}
\end{table}


% \begin{table}[]
% \begin{tabular}{l|c|c|c|c|c|c|c|c}
% \hline
%                 &Res152 &WRN  &DN201 &ViT-L &T2T-24 & TnT  & ViT-S & T2T-7 \\ \hline
% VGG19$_{bn}$    & 0.29 & 0.40 & 0.61 & 0.11 & 0.15 & 0.16  & 0.12  & 0.29  \\ \hline
% MNAS            & 0.42 & 0.40 & 0.76 & 0.11 & 0.27 & 0.26  & 0.21  & 0.63  \\ \hline
% DeiT-T          & 0.22 & 0.19 & 0.33 & 0.74 & 0.49 & 1.70  & 20.44 & 1.24  \\ \hline
% DeiT-T-RE       & 0.50 & 0.50 & 1.12 & 3.08 & 1.09 & 6.46  & 55.21 & 6.12  \\ \hline
% DeiT-S          & 0.20 & 0.19 & 0.31 & 0.67 & 0.73 & 2.45  & 8.31  & 0.81  \\ \hline
% DeiT-S-RE       & 0.89 & 0.93 & 2.05 & 4.90 & 3.57 & 21.56 & 64.65 & 10.59 \\ \hline
% DeiT-B          & 0.23 & 0.21 & 0.35 & 0.60 & 0.71 & 1.89  & 4.14  & 0.62  \\ \hline
% DeiT-B-RE       & 1.13 & 1.22 & 2.65 & 3.59 & 3.45 & 17.55 & 44.63 & 9.89  \\ \hline

% \end{tabular}
% \caption{Targetted Attack MIM at 16 EPS}
% \label{tbl:targetted_mim}
% \end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

